iLQGames.jl: Rapidly Designing and Solving Differential Games in Julia

In many problems that involve multiple decision making agents, optimal choices for each agent depend on the choices of others. Differential game theory provides a principled formalism for expressing these coupled interactions and recent work offers efficient approximations to solve these problems to non-cooperative equilibria. iLQGames.jl is a framework for designing and solving differential games, built around the iterative linear-quadratic method. It is written in the Julia programming language to allow flexible prototyping and integration with other research software, while leveraging the high-performance nature of the language to allow real-time execution. The open-source software package can be found at https://github.com/lassepe/iLQGames.jl.

==> Makefile <==
# config
MAIN=main
BIB=main.bib
# this must be always at least "." (otherwise things might be written to "/")
OUTDIR=../build

# Variables for later use
TEXFILES=$(shell find . -name "*.tex")
MAINDOCPATH=$(OUTDIR)/$(MAIN).pdf

# generic compilation setup
all: dirsetup $(MAINDOCPATH)

$(MAINDOCPATH): $(TEXFILES) $(BIB)
	latexmk -outdir=$(OUTDIR) -pdf $(MAIN).tex

dirsetup:
	# reproduce dir structure
	if [ ! -z "$(OUTDIR)" ]; then \
		texdirs=$$(find . -name "*.tex" | sed -r 's|/[^/]+$$||' | sort | uniq); \
		for d in $$texdirs; do mkdir -p $(OUTDIR)/$$d ; done \
	fi

clean:
	latexmk -outdir=$(OUTDIR) -CA

clean_all:
	rm -r ./$(OUTDIR)

.PHONY: all diresetup clean clean_all

